Mechanizing Refinement Types (extended)

Practical checkers based on refinement types use the combination of implicit semantic sub-typing and parametric polymorphism to simplify the specification and automate the verification of sophisticated properties of programs. However, a formal meta-theoretic accounting of the soundness of refinement type systems using this combination has proved elusive. We present \lambda_RF a core refinement calculus that combines semantic sub-typing and parametric polymorphism. We develop a meta-theory for this calculus and prove soundness of the type system. Finally, we give a full mechanization of our meta-theory using the refinement-type based LiquidHaskell as a proof checker, showing how refinements can be used for mechanization.

==> Makefile <==
all: pdf

pdf:
	latexmk -pdf main.tex

cont: continuous
continuous:
	latexmk -pvc -pdf -interaction=nonstopmode main.tex

chop:
	rm -f anon-supplemental.pdf anon-submission.pdf
	cp main.pdf anon-supplemental.pdf
	if which cpdf; \
         then cpdf  anon-supplemental.pdf "1-28" -o anon-submission.pdf; \
         else pdftk anon-supplemental.pdf cat 1-28 output anon-submission.pdf; fi

plain:
	touch no-editing-marks
	$(MAKE) clean
	$(MAKE) 

ed:
	rm -f no-editing-marks
	$(MAKE) clean
	$(MAKE)

clean:
	latexmk -c main.tex

cleanall:
	latexmk -C -bibtex main.tex

.PHONY: all pdf clean cleanall cont continuous plain ed


==> eval.tex <==
\section{Evaluation}
\label{sec:eval}
\begin{table}
  \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
    \hline
    \multirow{2}{*}{\diagbox{\footnotesize{Case Study}}{\footnotesize{Tool}}} & \multicolumn{4}{l|}{\toolname} & \multicolumn{2}{l|}{\mochi~\cite{unno_automating_2013}} & \multicolumn{2}{l|}{F* Implicits~\cite{fstar-implicits}} \\
    \cline{2-9}
    & SLOC & Time (s) & Specify & Verify & Specify & Verify & Specify & Verify \\
    \hline
    \textsc{incr}                     & 8    & 0.01  & \cmark & \cmark & \cmark & \xmark & \cmark & \xmark \\
    \textsc{sum}                      & 5    & 0.01  & \cmark & \cmark & \cmark & \cmark & \cmark &  \xmark \\
    \textsc{repeat}                   & 86   & 0.28  & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark \\
    $d_2$~\cite{unno_automating_2013} & 8    & 0.07  & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark \\
    \hline
    \multicolumn{6}{l}{\textbf{Resources}} \\
    \hline
    \textsc{incrState}                & 28   & 0.65  & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
    \textsc{accessControl}            & 49   & 0.36  & \cmark & \cmark & \cmark & \xmark & \cmark & \cmark\footnotemark \\
    \textsc{tick}~\cite{liquidate}    & 85   & 0.03  & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark \\
    \textsc{linearDSL}                & 20   & 0.03  & \cmark & \cmark & \xmark  & \xmark & \cmark & \cmark\footnotemark[1] \\
    \hline
    \multicolumn{6}{l}{\textbf{State Machines}} \\
    \hline
    \textsc{pagination}                              & 79   & 0.3    & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
    \textsc{login}~\cite{BradyStateMachinesAll2016}  & 121  & 0.09   & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
    \textsc{twoPhase}                                & 135  & 0.86   & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
    \textsc{tickTock}                                & 112  & 0.14   & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
    \textsc{tcp}                                     & 332  & 115.73\footnotemark[2] & \cmark & \cmark & \xmark  & \xmark & \xmark & \xmark \\
    \hline
  \end{tabular}
  \caption{Comparison of systems: \cmark indicates that the specification can be written or that the necessary implicit parameters for verification are instantiated, respectively.}
  \label{tab:eval}
\end{table}

We implement our system of Implicit Refinement Types in a tool dubbed \toolname, evaluate our tool using a set of illustrative examples and case studies, and compare our tool against the existing state of the art.
We aim to answer the following questions about Implicit Refinement Types and how they compare to the state of the art in implicit parameters:
\begin{description}
  \item[Q1:] Do Implicit Refinement Types enable \emphbf{lightweight verification} of higher-order functional programs? Is the theory-agnostic instantiation procedure sufficient to verify programs with Implicit Refinement Types, even without using heavyweight instantiation techniques such as domain-specific solvers and synthesis engines?
  \item[Q2:] Relative to the state of the art, are Implicit Refinement Types \emphbf{more expressive}? That is, can we use implicits to encode specifications that would've otherwise required the use of additional language features?
  \item[Q3:] Relative to the state of the art, are Implicit Refinement Types \emphbf{more flexible}? That is, do they allow \emph{automated verification} in places where unification-based implicits and CEGAR-based extra parameters do not?
\end{description}

\footnotetext{\label{fn:fstar}Verification requires annotating a simple fact about sets as \fstar does not include a native theory of sets.}
\footnotetext[2]{The tcp example blows up due to an asymptotically unoptimized congruence closure implementation in our prototype.}

\mypara{Implementation}
\label{sec:eval:implementation}
%
\toolname extends the language presented in \secref{sec:lang} with polymorphism
and type constructors and omits concrete syntax for implicit lambdas and
unpacks.
%
Instead, implicit parameters appear solely in specifications---that is,
refinement \emph{types}---and do not require implementation changes to the code.

Inserting implicit lambdas is straightforward: when checking
that a term has an implicit function type, insert a corresponding implicit
lambda.
%
Inserting implicit unpacks is more interesting: we need to unpack any term of
implicit pair type before we use it.
%
For instance, if $e$ has the type $\tcoifun{x}{t_1}{t_2}$,
then we must unpack $e$ to extract the
corporeal ($t_2$) component of the pair before we can apply a function to it:
$\app{e_f}{e}$ becomes $\eunpack{x}{y}{e}{\app{e_f}{y}}$.
%
To automate this procedure, we use an \textsc{Anf}-like
transformation.
%
However, instead of a full \textsc{Anf} transformation, \toolname only
A-normalizes terms of implicit pair type, replacing their use with a projection into the second
component of the pair ($y$ in the above term), and a binder for the first component ($x$).
%
This transformation ensures that the ghost parameter representing the
implicit component ($x$ in the above term) is in context where the implicit pair
is used.

Besides the above elaborations, we implement base type checking, constraint
generation using the algorithm from \secref{sec:constraint-generation}, and
solving using the theory-agnostic algorithm described in
\secref{sec:solving:special-case}.
%
The resulting VCs are checked using the Z3 SMT solver.

\mypara{Comparsion}
\label{sec:eval:comparison}
We compare \toolname to two other systems: the higher-order model checker
\mochi~\cite{unno_automating_2013}, and the
F* programming language's support for implicit parameters\footnote{%
% 
Note that F*'s main verification mechanism is Dijkstra Monads~\cite{Swamy:2013}, which we do not compare against in our evaluation.
% 
We discuss trade offs between Dijkstra Monads and Implicit Refinement Types in \secref{sec:related}.
}~\cite{fstar, fstar-implicits}.
%
Both systems, like \toolname and unlike foundational verifiers
 such as Idris~\cite{brady_idris_2013} and Coq~\cite{the_coq_development_team_coq_2009}, are
designed for lightweight, automatic verification.
%
\mochi aims to provide complete verification of higher-order programs by
automatically inserting extra (implicit) parameters.
%
Whereas \toolname has users write refinement type specifications (with
\emph{explicit} reference to implicit types), \mochi's specifications are implemented as
assertions within the code.
%
F*'s type system is a mix of a Martin-L\"of style dependent type system with
SMT-backed automatic verification of refinement type specifications.
%
Though there is no formal specification of implicit parameters in F*, they are
described as being implemented by unification~\cite{fstar-implicits} and
therefore are integrated as part of the Martin-L\"of side of the type system,
in contrast to how Implicit Refinement Types in \toolname fully integrate
refinement and implicit types.

%\mypara{Comparison with Existing Approaches}
%
% Auto-active verifiers like \toolname require 
% modular specifications, and hence straddle  
% the line between theorem proving and
% automatic verification.

Our comparison, summarized in \tabref{tab:eval}, consists of a series of
illustrative case studies that demonstrate the specifications that can be written in
each system (the Specify column) and whether they can find the necessary
implicit parameter instantiations (the Verify column).
%
As all three tools are designed to be used for lightweight verification, we
write the implementation and then separately write the specifications.
%
We do not rewrite the implementations to better accommodate specifications,
though for \mochi we insert assertions within the code as necessary to express
specifications.
%
(Link to full versions are elided for DBR.)

\subsection{Q1: Lightweight Verification}

First, we evaluate whether implicit refinements allow
users to write modular specifications that would otherwise 
be inexpressible with plain refinement types, via a series 
of higher-order programs that use implicits for lightweight 
verification.
%
The programs are designed to capture core aspects of 
various APIs and how Implicit Refinement Types permit specifications 
that can be automatically verified in a representative 
client program using the API.
%
Notably, for all of these examples \toolname only 
uses the theory-agnostic instantiation procedure 
from \secref{sec:solving:special-case} and does not
employ heavyweight instantiation techniques such 
as domain-specific solvers or synthesis engines.

\mypara{Higher-Order Loops}
%
Our first example, \textsc{repeat}, defines a 
stateful loop combinator \ha{repeat} that takes 
an increasing stateful computation \ha{body} 
and produces a stateful computation that loops 
\ha{body} \ha{count} times.
% 
Its signature in \toolname is:
% 
\begin{code}
  repeat :: body:([x:Int] -> ([y:{v:Int | v > x}]. SST x y Int Int))
         -> count:{v:Int | v > 0}
         -> ([q:Int] -> ([r:{v:Int | v > q}]. SST q r Int Int))
\end{code}
% 
which says that the input and output are a stateful computations whose history
and prophecy variables together guarantee that the computation will leave the
state larger than it started.
% 
In the first line the implicit function argument \ha{x} is externally determined
and captures the state of the world before the \ha{body} computation, while the
implicit pair component \ha{y} captures that \ha{body} updates the state of the
world to some (unknown) larger value.

The implicit pairs are necessary to specify \ha{repeat},
as the updated state is determined by an internal choice 
in \ha{body}.
%
\textsc{repeat} also demonstrates how implicit pairs can 
specify loop invariants (here upward-closure) on higher-order 
stateful programs.
%
Though \ha{repeat} is specified using implicit pairs, 
\toolname does \emph{not} require that arguments passed 
to \ha{repeat} be specified using implicit pairs.
%
In \textsc{repeat} we define a function \ha{incr} with 
the type \ha{[x:Int] $\rightarrow$ SST x (x + 1) Int Int} 
that increments the state.
%
\toolname will appropriately type check and verify \ha{repeat incr}
as Implicit Refinement Types automatically account for the necessary subtyping 
constraints to ensure that \ha{incr} meets the conditions of \ha{repeat}.

\mypara{State Machines}
%
The next set of examples demonstrate that Implicit Refinement Types 
let us specify and verify state-machine based protocols
that are ubiquitous, spanning appications from  
networking protocols to device driver and operating 
system invariants~\cite{BradyStateMachinesAll2016}.
%
IRTs\MK{We should use ``IRTs''/``Implicit Refinement Types'' or ``Implicits'', not both.} let us encode state machines as transitions 
allowed from a ghost state using the Hoare State Monad 
developed in \secref{sec:overview:state}.

\textsc{login} from \citet{BradyStateMachinesAll2016}, 
which models logging into a remote server, served as our 
initial inspiration for studying this class of problems.
We verify that a client respects the sequence of 
connect, login, and only then access information.

\textsc{tickTock} verifies that two \ha{ticker} and
\ha{tocker} processes obey a state machine for 
the tick-tock example standard to the concurrency 
literature~\cite{scalas_verifying_2019}.
%
Here we show the implementation of \ha{tocker}.
\begin{code}
  tocker = \c -> do
    msg <- recv c
    if msg = tick then send c tock else assert False
\end{code}
Ghost parameters on \ha{send} and \ha{recv} track 
the state machine and ensure messages follow the 
tick-tock protocol.
%
If \mbox{\ha{send c tock}} is changed to \mbox{\ha{send c tick}}
the program is appropriately rejected.

\textsc{twoPhase} is a verified implementation of 
one side of a two-phase commit process. 
%
This example serves as a scale model for \textsc{tcp}, 
a verified implementation of a model of a TCP client 
performing a 3-way handshake, using the TCP state 
machine\cite{RFC0793}.

\textsc{pagination} is an expanded version of our 
stream example from \sectionref{sec:overview}, and 
models the AWS S3 pagination API~\cite{RetrievingPaginatedResults}.
%
This example shows that our protocol state machine 
need not be finite, as it is specified with respect 
to an \emph{unbounded} state machine.
% \footnote{Indeed, using this style we can encode protocol state machines
% given by any provably-terminating Turing machine, where the type-level
% computation is performed automatically by \emph{Logical
% Evaluation}\cite{vazou_refinement_2018}}

\mypara{Quantitative Resource Tracking}
%
The next set of examples reflect various patterns 
of specifying and verifying \emph{resources} and 
demonstrate that Implicit Refinement Types enable
lightweight verification of these patterns.
%
The examples show how \toolname handles specification 
and automatic verification when dealing with resources 
such as the state of the heap and quantitative
resource usage.
%
In \secref{subsec:examples:grant} we saw how Implicits enable
specifying the access-control API from \figref{fig:revoke}; 
the \textsc{accessControl} example verifies clients of this API.
%
In contrast, \textsc{tick} (as shown in \secref{subsec:tick}) follows
\citet{liquidate} in defining an applicative functor that tracks resource usage.
% 
The key distinction from \citet{liquidate} 
is that the resource count exists only at 
the type level.
%
This example generalizes: we can port any of 
the \emph{intrinsic verification} examples 
from that work to use implicit parameters 
instead of explicitly passing
around resource bounds.
% \footnote{
% In fact, using implicit parameters, we can also ``interalize'' their heavyweight
% \emph{extrinsic verification} examples, and write these types in the
% \emph{intrinsic} style.
% %
% In this case, we still require the same
% refinement-reflection-based proofs.}

\textsc{linearDSL} embeds a simple linearly typed DSL in \toolname.
% 
It allows us to embed linear terms in \toolname, with linear
usage of variables statically checked by our refinement type system.
%
The syntactic constructs of this DSL are smart constructors that take the typing
environments as implicit parameters, enforcing the appropriate linear typing
rules.

\toolname enables specification and automatic verification of this diverse range
of examples, and in fact only requires the theory-agnostic instantiation
procedure to find the correct implicit instantiations.
%
This demonstrates that Implicit Refinement Types enable lightweight
verification of a variety of higher-order programs, and that they are
widely useful even without a domain specific solver or heavyweight 
synthesis algorithm.

\subsection{Q2: Expressivity}

We compare the expressivity of Implicit Refinement Types as implemented in
\toolname to the assertion-based verification of \mochi and the implicit
parameters of \fstar. 
%
First, merely the fact that we allow users to explicity write specifications
using implicit parameters allows us to write specifications we otherwise
could not. In particular, this is witnessed by the \textsc{tick} and
\textsc{linearDSL} examples that specify resource tracking, a
non-functional property. \mochi cannot express the specifications
for these because there is no combination of program variables that
computes the (non-functional) \emph{usage} properties used in these specifications.

Second, Implicit Pair Types add expressivity by allowing us to write
specifications against choices made \emph{internal} to functions that we
wish to reason about.
%
For example, \textsc{repeat} uses implicit pairs to specify 
a loop invariant. 
%
This example can't be done with \fstar's implicits, as, absent
implicit pairs, we cannot bind to the return value of the loop 
body.
%
As a result, in \fstar we cannot verify this example with 
implicits alone: we would have to bring in additional 
features such as the Dijkstra monad~\cite{Swamy:2013}.

Similarly, \emph{none} of the protocol state machine examples 
can be encoded with implicit functions alone. Implicit pairs 
are required to write specifications against choices made by 
other actors on the protocol channel. 
%
As a result, these examples also cannot be encoded 
in \fstar's implicits. These state machine specifications 
cannot even be expressed in \mochi as they crucially 
require access to ghost state, which \mochi does not support.

\subsection{Q3: Flexibility}

\begin{figure}[t!]
\begin{code}
incr :: [n:Int] -> (Int -> SInt n) -> SInt (n + 1)
incr f = (f 0) + 1

test1 :: SInt 11                test2 :: m:Int -> SInt (m + 1)
test1 = incr (\x -> 10)         test2 m = incr (\x -> m)
\end{code}
\caption{A higher order increment function}
\label{fig:incr}
\end{figure}
 
We compare the flexibility that our refinement-integrated 
approach gives us to solve for implicit parameters
relative to that of other systems.
%
We focus on the features of our semantics and
our abstract solving algorithm from~\sectionref{sec:solving:together} 
independently of the choice of quantifier
elimination procedure, which we examined above.
%
We illustrate these differences with several examples.
%
\textsc{incr} is the program from Figure~\ref{fig:incr}.
In \mochi the specification is given by assertions that 
\ha{test1} and \ha{test2} are equal to \ha{11} and \ha{m + 1} 
respectively.
%
\textsc{incrState} generalizes \textsc{incr} to track 
the integer in the singleton state monad instead of a 
closure.
%
\textsc{sum} is similar to \ha{incr} except that it takes 
two implicit arguments and two function arguments, returning 
the sum of the two returned values:
  %
\begin{code}
  sum :: [n:Int, m:Int] -> (Int -> SInt n) -> (Int -> SInt m) -> SInt (n + m)
  sum f g = (f 0) + (g 0)
  
  test :: SInt 11
  test = sum (\x -> 10) (\y -> 1)
\end{code}
%
All three tools can specify the program. 
%
\toolname and \mochi successfully instantiate 
the implicit parameters needed for verification.
%
\textsc{D2} is an example from the 
\mochi~\cite{unno_automating_2013} 
benchmarks that loops a nondeterministic 
number of times and adds some constant each time.
%
Unlike \toolname, \mochi is unable 
to solve \textsc{accessControl}, as 
CEGAR is notoriously brittle on 
properties over the theory of 
set-operations.

\mypara{Comparsion to \mochi}
%
The results of the comparison to \mochi are summarized in Table~\ref{tab:eval}
%
%%%INCR
\mochi fails to automatically verify \textsc{incr}, 
but it succeeds if either \ha{test1} or \ha{test2} 
appear individually.
%
This is partly due to the unpredictability of \mochi's 
CEGAR loop~\cite{JhalaMcMillan06}, as it suceeds in 
verifying \textsc{incrState}.
%INCR
Additionally, \mochi attempts to infer specifications
(including adding implicit arguments to functions) 
\emph{globally}.
%
This can lead to the anti-modular behavior seen here.
%
In contrast, by introducing implicit arguments 
as a user-level specification technique, \toolname 
permits modular verification. 
%
The existence of \ha{test1} has no effect on 
the verification of \ha{test2}, as we generate
two separate quantifier instantiation problems 
that \toolname solves locally.

In the example \textsc{D2}, \toolname \emph{fails} 
to solve the existential constraints generated by 
implicit instantiation as that requires solving 
systems of inequalities, which our theory-agnostic 
quantifier elimination does not attempt.
%
However, \toolname captures the full set of constraints 
and could, with a theory specific solver like \mochi's, 
verify \textsc{D2}.
%
Concretely, \textsc{D2} yields a constraint 
of the form $\exists x. true \Rightarrow x > 3$, 
which  could be discharged by instantiating the 
abstract algorithm of \sectionref{sec:solving}
with either the solver from \mochi\cite{unno_automating_2013} 
or EHSF\cite{RybalchenkoEHSF}, or by composing 
them using the algorithm from \secref{sec:solving:special-case}.
%
%That is, Implicit Refinement Types can make use of other 
%solvers that operate on exists-forall constraints, such those for 
%arithmetic inequalities\cite{unno_automating_2013}---which would solve this particular 
%constraint---or even synthesis engines like Synquid\cite{polikarpova_program_2016}, described in \sectionref{sec:related}.

\mypara{Comparsion to Unification}
%
The results of the comparison to \fstar's unification-based implicits are
summarized in Table~\ref{tab:eval}.
%
Implicit Refinements are more flexibile as \fstar attempts to solve the
implicits purely through unification, \ie without accounting for refinements. In
contrast, \toolname generates subtyping (implication) constraints that are
handled separately from unification.
% 
% Instantiation with unification generates 
% \emph{local unification constraints}, whereas 
% Implicit Refinement Types generate EHCs that 
% capture \emph{global subtyping constraints}, 
% allowing for reasoning in context.
%
%
When the unification occurs under a type 
constructor, then unification succeeds.
%
For example, \fstar verifies \textsc{incrState}
because elevating the ghost state to a parameter 
of the singleton state type constructor makes 
it ``visible'' to \fstar's unification algorithm.
%
However, if there is \emph{no} type constructor
to guide the unification, \fstar must rely on
higher-order unification, which is undecidable 
in general and difficult in practice.
%%INCR
For this reason, in the \textsc{incr} example 
from Figure~\ref{fig:incr}, \fstar fails to 
instantiate the implicit arguments needed to 
verify \ha{test1} and \ha{test2}, even if we 
aid it with precise type annotations on 
\ha{\x $\rightarrow$ 10} and \ha{\x $\rightarrow$ m}, and
%%SUM
\fstar fails to verify the \textsc{sum} example 
for the same reason.
%
By contrast, \toolname can take advantage 
of the refinement information to successfully 
solve for the implicit parameters. 
%
%%d2
Finally \fstar's unification fundamentally 
cannot handle an example like \mochi's 
\textsc{D2}, as unification will not be 
able to find an implicit instantiation
when it is only constrained by inequalities.



==> javaListings.tex <==
\def\codesize{\normalsize}
% \def\codesize{\footnotesize}
\def\incodesize{\normalsize}

\lstdefinelanguage{myjava}{  
  basicstyle=\ttfamily\codesize,        % the size of the fonts that are used for the code
  backgroundcolor=\color{white},   % choose the background color
  basicstyle=\codesize\tt,        % size of fonts used for the code
  breaklines=true,                 % automatic line breaking only at whitespace
  captionpos=b,                    % sets the caption-position to bottom
  morecomment=[l][\color{gray}\itshape\codesize]{//},
  %morecomment=[s][\ttfamily\itshape\codesize]{/*}{*/}
  %commentstyle=\color{mygreen},    % comment style
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  keywordstyle=\color{red},       % keyword style
  stringstyle=\color{mymauve},     % string literal style
  escapeinside={(*}{*)},
  emphstyle={[1]\bfseries\color{black}},
  emphstyle={[2]\color{violet}},
  emphstyle={[3]\color{teal}},
  emphstyle={[4]\color{blue}},
  emph=
  {[1]
   public,static,var,return
  },
  emph=
  {[2]
   void,String,Obj,int
  },
  emph=
  {[3]
   source,sink,new
  },
  emph=
  {[4]
   ex1,smash,put,get,set,setGet,putGet,baz,ex2,ex2a,ex2b,ex3
  },
}

\colorlet{shadecolor}{gray!10}

\lstnewenvironment{javacode}
{\lstset{language=myjava,linebackgroundcolor={\ifodd\value{lstnumber}\color{shadecolor}\fi}}}
{}

\def\mcode{\lstinline[language=myjava,basicstyle=\ttfamily\incodesize,mathescape=true]}
